OPPO: Accelerating PPO-based RLHF via Pipeline Overlap

Proximal Policy Optimization (PPO)-based reinforcement learning from human feedback (RLHF) is a widely adopted paradigm for aligning large language models (LLMs) with human preferences. However, its training pipeline suffers from substantial inefficiencies due to sequential multi-model dependencies (e.g., reward model depends on actor outputs) and long-tail response lengths, where a few long responses straggle the stage completion. We present OPPO, a novel, lightweight, and model-agnostic PPO-based RLHF framework that improves training efficiency by overlapping pipeline execution. OPPO introduces two novel techniques: (1) Intra-step overlap, which streams upstream model outputs (e.g., actor model) in right-sized chunks, enabling the downstream model (e.g., reward) to begin prefill while the upstream continues decoding; and (2) Inter-step overlap, which adaptively overcommits a few prompts and defers long generations to future steps, mitigating tail latency without discarding partial work. OPPO integrates easily with existing PPO implementations with a lightweight wrapper. Extensive evaluations show that OPPO accelerates PPO-based RLHF training by $1.8\times$--$2.8\times$ and improves GPU utilization by $1.4\times$--$2.1\times$ without compromising training convergence.

==> Section/10_Proof.tex <==
\section{Theoretical Analysis}


This section proves that \name\ (i) preserves the statistical correctness of
PPO, (ii) cannot lengthen---and typically shortens---the critical path of one
iteration, (iii) still converges when a small fraction of samples is deferred
by \emph{inter-iteration overlap}, and (iv) guarantees a positive throughput
gain whenever responses exhibit long-tail latency.  Each lemma is followed by
an informal explanation of \emph{why} the claim holds.


\subsection{Unbiasedness of the streamed policy-gradient estimator}


We first show that streaming tokens to the reward and critic models has no
effect on the expected PPO update.

Consider the actor be $\pi_\theta(\cdot \mid x)$, a prompt be
$x\!\sim\!\mathcal D$, and a full response be
$y=(y_1,\dots,y_L)\!\sim\!\pi_\theta$.  While decoding, the system produces a
sequence of prefixes
$y^{(1)},\dots, y^{(T)}$ with $y^{(T)}\!=\!y$.
The advantage computed on the \emph{final} string is
$\widehat A(y)$.

\paragraph{Streamed estimator.}
Only the \emph{last} prefix contributes to the gradient, as captured by the
indicator $\mathbf 1_{\mathrm{fin}}^{(i,t)}$:

\[
\widehat{\mathbf g}_{\mathrm{str}}(\theta)
  = \frac{1}{B} \sum_{i=1}^{B}
    \sum_{t=1}^{T_i}
    \mathbf 1_{\mathrm{fin}}^{(i,t)}\,
    \widehat{A}(y_i)\,
    \nabla_\theta\!\log\pi_\theta(y_i \mid x_i).
\]
Where the $\mathbf 1_{\mathrm{fin}}^{(i,t)} = 1$ if $t = T_i$ and 0 otherwise. 

\paragraph{Standard estimator.}
The textbook PPO estimator is

\[
\widehat{\mathbf g}_{\mathrm{std}}(\theta)
  = \frac{1}{B} \sum_{i=1}^{B}
    \widehat{A}(y_i)\,
    \nabla_\theta\!\log\pi_\theta(y_i \mid x_i).
\]

\paragraph{Proof.}
Because exactly one prefix per sample is final,
$\sum_{t}\mathbf 1_{\mathrm{fin}}^{(i,t)}=1$.  The inner sum therefore
collapses, making $\widehat{\mathbf g}_{\mathrm{str}}(\theta)$ algebraically
identical to $\widehat{\mathbf g}_{\mathrm{std}}(\theta)$.  Two random
variables that coincide point-wise share the same expectation and variance:
\[
\mathbb E[\widehat{\mathbf g}_{\mathrm{str}}]
  =\mathbb E[\widehat{\mathbf g}_{\mathrm{std}}],
  \qquad
\operatorname{Var}[\widehat{\mathbf g}_{\mathrm{str}}]
  =\operatorname{Var}[\widehat{\mathbf g}_{\mathrm{std}}].
\]


\subsection{Critical-path speed-up from intra-step overlap}


\paragraph{Timing notation.}
\[
T_{\mathrm{sync}} = G + P + R,
\qquad
T_{\mathrm{stream}} = \max\!\{\,G,\;P+R\,\}.
\]

Here $G$ is actor decode time, $P$ is reward/critic pre-fill, and
$R$ is the residual scoring time.

\paragraph{Claim.}
\[
T_{\mathrm{stream}}\le T_{\mathrm{sync}},
\qquad
\frac{T_{\mathrm{sync}}}{T_{\mathrm{stream}}}
  \ge 1 + \frac{\min\{G,P\}}{T_{\mathrm{sync}}}.
\]

\paragraph{Proof.}
\emph{Case~1} When($G\!\ge\!P+R$):
$T_{\mathrm{stream}}\!=\!G$ and the time saved is $P+R\!\ge\!P$.  
\[
\frac{T_{\mathrm{sync}}}{T_{\mathrm{stream}}}
   = 1 + \frac{P+R}{G}
   \ge 1 + \frac{P}{T_{\mathrm{sync}}}.
\]

\emph{Case~2} When ($P+R\!\ge\!G$) is symmetric, saving exactly $G$.  At least the
shorter of $G$ and~$P$ disappears from the critical path.

Sequential pipelines add stage times; overlapping
pipelines take the maximum.  The smaller stage is therefore “free’’
after streaming.



\subsection{Convergence with one-step deferral}


Over-commitment can defer up to $\delta$ responses by one iteration.  We model
that as adding a bounded, one-step-old gradient term.

\paragraph{Update rule.}
\[
\theta_{k+1}
  = \theta_k - \eta\bigl(\mathbf g_k + \mathbf d_k\bigr),
\qquad
\|\mathbf d_k\|_2 \le D_{\max}.
\]

\paragraph{Assumptions.}
The surrogate loss $\mathcal L$ is $\mu$-strongly convex and
has $L$-Lipschitz gradient; $\|\mathbf g_k\|_2\!\le\!G_{\max}$.

\paragraph{Bound.}
For $\eta\!\le\!1/(L+\mu)$,
\[
\mathbb E\!\bigl[\|\theta_k - \theta^\star\|_2^2\bigr]
  \le (1-2\eta\mu)^k\|\theta_0 - \theta^\star\|_2^2
     + \frac{4\eta^2 D_{\max}^2}{\mu}.
\]

\paragraph{Proof sketch with details.}
Expanding
$\|\theta_{k+1}-\theta^\star\|_2^2$,
taking conditional expectation, using strong convexity for the descent term
and Cauchy–Schwarz for the variance term yields a contraction factor
$(1-2\eta\mu)$ plus an $O(\eta^2 D_{\max}^2)$ bias.  Full derivations follow
delayed-SGD analyses such as \citet{recht2011hogwild}.

Deferring by one step is mathematically the same as adding a
bounded noise vector; with small learning rates, its long-run effect
shrinks with~$\eta^2$.

\todo{Here I think we should have weaker assumptions like the smoothness, because it can be shown by our stalness graph, So it need to update.}


\subsection{Throughput guarantee from over-commit}


Finally we connect deferral to end-to-end samples-per-second.

\paragraph{Random variables.}
\[
\mathbb E[T_{\mathrm{sync}}]
  = T_{\mathrm{fast}} + p\,\Delta_{\mathrm{slow}},
\qquad
T_{\method} = T_{\mathrm{fast}}.
\]

\paragraph{Speed-up.}
\[
\mathrm{Speed\text{-}up}
  = \frac{\mathbb E[T_{\mathrm{sync}}]}{T_{\method}}
  = 1 + p\,\frac{\Delta_{\mathrm{slow}}}{T_{\mathrm{fast}}} > 1.
\]

\paragraph{Explanation.}
A synchronous batch waits for every response.  Whenever even one
straggler appears (probability~$p$), the baseline pays the full penalty
$\Delta_{\mathrm{slow}}$.  \name\ ignores stragglers and therefore never
incurs that cost.






% Generalized Advantage Estimation (finite-horizon)
\begin{equation}
\delta_t \;=\; r_t + \gamma V_\phi(s_{t+1}) - V_\phi(s_t), 
\qquad
\hat A_t \;=\; \sum_{\ell=0}^{T-t-1} (\gamma\lambda)^{\ell}\, \delta_{t+\ell}.
\end{equation}
% (Optional recursive form) \hat A_t = \delta_t + \gamma\lambda \hat A_{t+1},\; \hat A_T = 0.

% PPO clipped surrogate (maximize); behavior policy is \theta_{j-1}
\begin{align}
r_t(\theta_j) &= \frac{\pi_{\theta_j}(a_t \mid s_t)}{\pi_{\theta_{j-1}}(a_t \mid s_t)},\\
\mathcal{J}_{\text{clip}}(\theta_j) 
&= \mathbb{E}_{(s_t,a_t)\sim D_{\theta_{j-1}}}
\!\left[
\min\!\left(
r_t(\theta_j)\,\hat A_t,\;
\operatorname{clip}\!\big(r_t(\theta_j), 1-\epsilon, 1+\epsilon\big)\,\hat A_t
\right)
\right].
\end{align}
% If you prefer a loss to MINIMIZE:
\begin{equation}
\mathcal{L}^{\text{PPO}}(\theta_j) \;=\; -\,\mathcal{J}_{\text{clip}}(\theta_j).
\end{equation}

% (Optional) KL-shaped terminal reward often used in RLHF:
% \tilde r_t = 0 \text{ for } t<T,\quad
% \tilde r_T = r_{\text{RM}}(x,y) - \beta\,\mathrm{KL}\!\left(\pi_{\theta_{j-1}}(\cdot\mid x,y_{<T}) \,\|\, \pi_{\text{ref}}(\cdot\mid x,y_{<T})\right).

